Enhancing Adversarial Robustness via Test-time Transformation Ensembling

Deep learning models are prone to being fooled by imperceptible perturbations known as adversarial attacks. In this work, we study how equipping models with Test-time Transformation Ensembling (TTE) can work as a reliable defense against such attacks. While transforming the input data, both at train and test times, is known to enhance model performance, its effects on adversarial robustness have not been studied. Here, we present a comprehensive empirical study of the impact of TTE, in the form of widely-used image transforms, on adversarial robustness. We show that TTE consistently improves model robustness against a variety of powerful attacks without any need for re-training, and that this improvement comes at virtually no trade-off with accuracy on clean samples. Finally, we show that the benefits of TTE transfer even to the certified robustness domain, in which TTE provides sizable and consistent improvements.

==> tables/gaussian_filtering.tex <==
\begin{table}[]
\centering
\caption{\textbf{Using Gaussian filtering as a test-time transformation.} We test the impact in adversarial robustness of introducing a transformation that was \textit{not} seen during training. In particular, we introduce a Gaussian-filtered version of the image, and record robust accuracy. Introducing Gaussian transformations, unseen by the model at training time, is detrimental for adversarial robustness.}
\centering
\small
\begin{tabular}{l|l|l|c}
\hline
Method                          & Clean     & Robust & Diff.    \\
\hline\hline
TRADES                          & 84.92	    & 53.11  & -        \\ \hline
+ Gaussian ($k=3$, $\sigma=1$)  & 81.59     & 50.21  & -2.90    \\
+ Gaussian ($k=3$, $\sigma=2$)  & 81.27     & 49.63  & -3.48    \\ \hline
+ Gaussian ($k=5$, $\sigma=1$)  & 80.36     & 49.19  & -3.92    \\
+ Gaussian ($k=5$, $\sigma=2$)  & 76.78     & 45.71  & -7.40    \\ \hline
\end{tabular}
\label{tab:gaussian}
\end{table}

==> tables/intelligent_crops.tex <==
\begin{table}[]
\centering
\caption{\textbf{Smart crop selection based on spatial patterns.} We construct ensembles of crops based on the spatial patterns observed in Figure~\ref{fig:crops} and record differences in robust accuracy.}
\centering
\small
\begin{tabular}{l|l|l}
\hline
Method              & Clean     & Robust    \\ \hline\hline
TRADES              & xxxxx	    & xxxxx     \\ \hline
+ X crops (random)  & xxxxx     & xxxxx     \\
+ X crops (smart)   & xxxxx     & xxxxx     \\ \hline
\end{tabular}
\label{tab:smart}
\end{table}
